NetInfoF Framework: Measuring and Exploiting Network Usable Information

Given a node-attributed graph, and a graph task (link prediction or node classification), can we tell if a graph neural network (GNN) will perform well? More specifically, do the graph structure and the node features carry enough usable information for the task? Our goals are (1) to develop a fast tool to measure how much information is in the graph structure and in the node features, and (2) to exploit the information to solve the task, if there is enough. We propose NetInfoF, a framework including NetInfoF_Probe and NetInfoF_Act, for the measurement and the exploitation of network usable information (NUI), respectively. Given a graph data, NetInfoF_Probe measures NUI without any model training, and NetInfoF_Act solves link prediction and node classification, while two modules share the same backbone. In summary, NetInfoF has following notable advantages: (a) General, handling both link prediction and node classification; (b) Principled, with theoretical guarantee and closed-form solution; (c) Effective, thanks to the proposed adjustment to node similarity; (d) Scalable, scaling linearly with the input size. In our carefully designed synthetic datasets, NetInfoF correctly identifies the ground truth of NUI and is the only method being robust to all graph scenarios. Applied on real-world datasets, NetInfoF wins in 11 out of 12 times on link prediction compared to general GNN baselines.

==> 000abstract.tex <==
Given a node-attributed graph, can we tell whether the graph neural networks (GNNs) will perform better than multi-layer perception (MLP) on graph tasks? 
Graph tasks, such as link prediction and node classification, are commonly solved by adopting GNNs.
\xiangsx{What are graph tasks? Can we introduce graph tasks first, i.e., the second sentence then raise this question?}
% If so, what is the best way to improve the accuracy?
% GNNs are commonly adopted on graph data for performing downstream tasks such as link prediction and node classification. 
However, they may not always work as expected in some graph scenarios, for example, in the case that the structure is randomly connected. 
\xiangsx{What does structure is uniform mean?}
Figuring out the reasons is not trivial and can cost a huge amount of time and resources. 
That is to say, how can we identify the usable information in the graph data in a principled way?
To address this, we propose \method, including \analysis and \model, for the detection and the exploitation of network usable information, respectively.
Given a graph data, \analysis measures the network usable information (NUI) without any model training, and \model to solve link prediction and node classification, while two modules share the backbone.
\james{what tasks do we refer to? I cannot understand the NetInfoA\_Act\'s function purely based on this sentence}
In summary, \method has following notable advantages:
(a) \general, handling both link prediction and node classification;
(b) \principled, with theoretical guarantee and closed-form solution;
(c) \effective, with the highest average rank, thanks to the proposed adjusted node similarity;
\james{ may change this to our performance numbers}
\christos{YES! lets give our best few numbers!}
(d) \scalable, being linear with the input size.
Applied \method on both synthetic and real-world graphs, \analysis successfully identifies the ground truth usable information in the synthetic datasets, and \model always wins or ties with many GNN baselines.
Our success story further demonstrate the correctness of \analysis in a real-world scenario, where there is no usable information in graphs constructed with some specific types of edges.
